Glove2Hand: Synthesizing Natural Hand-Object Interaction from Multi-Modal Sensing Gloves

Understanding hand-object interaction (HOI) is fundamental to computer vision, robotics, and AR/VR. However, conventional hand videos often lack essential physical information such as contact forces and motion signals, and are prone to frequent occlusions. To address the challenges, we present Glove2Hand, a framework that translates multi-modal sensing glove HOI videos into photorealistic bare hands, while faithfully preserving the underlying physical interaction dynamics. We introduce a novel 3D Gaussian hand model that ensures temporal rendering consistency. The rendered hand is seamlessly integrated into the scene using a diffusion-based hand restorer, which effectively handles complex hand-object interactions and non-rigid deformations. Leveraging Glove2Hand, we create HandSense, the first multi-modal HOI dataset featuring glove-to-hand videos with synchronized tactile and IMU signals. We demonstrate that HandSense significantly enhances downstream bare-hand applications, including video-based contact estimation and hand tracking under severe occlusion.

==> assets/backup.tex <==

% \begin{table}[!htp]\centering
% \caption{Comparison on InterHand~\cite{moon2020interhand2} dataset}\label{tab:ablation-interhand}
% \begin{tabular}{lcccc}\toprule
% \textbf{Method} &\textbf{PSNR} $\uparrow$ &\textbf{SSIM} $\uparrow$ &\textbf{LPIPS} $\downarrow$ &\textbf{FPS} $\uparrow$ \\\midrule
% Livehand~\cite{mundra2023livehand} &\textbf{28.4} &0.912 &\textbf{0.045} &50 \\
% Ours &27.5 &\textbf{0.943} &0.062 &\textbf{160} \\
% \bottomrule
% \end{tabular}
% \end{table}



% We evaluate video quality using FID (Fréchet Inception Distance) for image quality, FVD (Fréchet Video Distance) for short video sequences, and FVD-long for extended temporal coherence. Additionally, we conduct human studies to assess perceptual quality and validate utility through downstream task performance.


\begin{table}[!htp]\centering
\caption{Generated by Spread-LaTeX}\label{tab: }
%\resizebox{ extwidth}{!}{ % use this if the table is too large
\begin{tabular}{lrrrrrrrrrrr}\toprule
\multirow{3}{*}{Task} &\multicolumn{5}{c}{Contact IoU (\%)} &\multicolumn{5}{c}{Precision / Recall (\%)} \\\cmidrule{2-11}
&\multicolumn{4}{c}{Ours} &\multirow{2}{*}{PressureVision} &\multicolumn{4}{c}{Ours} &\multirow{2}{*}{PressureVision} \\\cmidrule{2-5}\cmidrule{7-10}
&Hand only &Hand+G2H &G2H only &Glove only & &Hand only &Hand+G2H &G2H only &Glove only & \\\midrule
Open Bottle lid &86.9 &\textbf{89.4} &71 &62.6 &0 &90.5 / 95.7 &93.6 / 94.9 &82.7 / 83.4 &74.2 / 79.9 &7.9 / 0 \\
Rotate object in air &85.6 &\textbf{88.7} &83.3 &79 &0.1 &89.3 / 95.4 &\textbf{92.4 / 95.7} &94.2 / 87.8 &89.5 / 87.1 &20.8 / 0.1 \\
Pick and Place &54.6 &\textbf{57.2} &24.6 &21.9 &0 &75.7 / 66.2 &\textbf{78.9 / 67.5} &53.7 / 31.3 &34.8 / 37.2 &1.6 / 0 \\
Play Piano &88.2 &\textbf{91.9} &78.6 &77.6 &0.1 &92 / 95.6 &\textbf{93.7 / 97.7} &93.8 / 82.9 &85.3 / 89.6 &26.9 / 0.1 \\
Tap/Press/Slide Surface &\textbf{90.9} &90.2 &60.6 &68.8 &15.2 &95.7 / 94.8 &94.3 / 95.4 &95.9 / 62.2 &87.5 / 76.3 &83.6 / 15.7 \\
Overall &85.3 &\textbf{88.2} &75.6 &71.5 &0.8 &90 / 94.2 &\textbf{92.6 / 94.9} &90.6 / 82 &82.8 / 83.9 &62.5 / 0.9 \\
\bottomrule
\end{tabular}
\end{table}

==> assets/related_work.backup.nov13.tex <==
\section{Related Work}

% \textbf{Generative Models for Hands.} Research on generating hand imagery falls into three main categories. The first focuses on \textbf{hand avatars}~\cite{iwase2023relightablehands, dong2025handsplat, zheng2024ohta, karunratanakul2023harp, zhao2024gaussianhand, chen2023hand}. These methods reconstruct a 3D hand representation and use raytracing~\cite{braunig2023realistic}, NeRF~\cite{mildenhall2021nerf}, or Gaussian Splatting~\cite{kerbl20233d} to generate images. Their primary advantage is precise controllability over hand pose and viewpoint. However, they are typically limited to generating the hand in isolation (``in-air''), lacking the ability to synthesize realistic backgrounds or detailed hand-object interactions.

% The second direction explores \textbf{hand diffusion models}~\cite{chen2025foundhand, pelykh2024giving, lu2024handrefiner, narasimhaswamy2024handiffuser, park2024attentionhand, zhang2025hand1000, MANO}. These works address the challenge of generating physically plausible hands within general image synthesis pipelines. Unlike avatar-based methods, they can produce images with backgrounds and object interactions. Their limitations include lacking precise pose control, the hand often being a small part of the overall generation (lacking detail), and a primary focus on single images rather than coherent video sequences depicting action.

% The third category is \textbf{hand-object interaction synthesis}~\cite{ye2023affordance, xu2023interdiff, zhang2024hoidiffusion}.  Unlike hand diffusion models, these methods specialize in generating close-up, detailed images of hand-object contact. For example, AffordanceDiffusion~\cite{ye2023affordance} estimates a grasp pose from an object image and synthesizes a hand grasping the object. HOIDiffusion~\cite{zhang2024hoidiffusion} renders images from interacting hand and object meshes.

% Our framework is distinguished from these lines of work in two key aspects: (1) We generate videos of hand-object interaction, capturing dynamic actions rather than static images. (2) The hand motions are grounded by an input glove video. This physical grounding enables scalable data curation by not relying on object meshes (difficult to obtain for non-rigid objects); it offers precise controllability, as the generated video is directly driven by a customizable glove recording; and it facilitates the fusion of hand videos and other sensing modalities from the data glove.

\textbf{Generative Models for Hands.} Research on generating hand imagery falls into three main categories. \textbf{Hand avatars}~\cite{iwase2023relightablehands, dong2025handsplat, zheng2024ohta, karunratanakul2023harp, zhao2024gaussianhand, chen2023hand} use rendering methods like raytracing~\cite{braunig2023realistic}, NeRF~\cite{mildenhall2021nerf} or Gaussian Splatting~\cite{kerbl20233d, braunig2023realistic} to offer precise pose and viewpoint control, but are typically limited to generating the ``in-air'' hand, lacking backgrounds or interaction. \textbf{Hand diffusion models}~\cite{chen2025foundhand, pelykh2024giving, lu2024handrefiner, narasimhaswamy2024handiffuser, park2024attentionhand, zhang2025hand1000, MANO} generate plausible hands within general image synthesis pipelines, including backgrounds, but lack precise control and focus on single, often low-detail, static images. Finally, \textbf{hand-object interaction synthesis}~\cite{ye2023affordance, xu2023interdiff, zhang2024hoidiffusion} specializes in generating close-up, static images of contact, for instance by estimating a grasp from an object~\cite{ye2023affordance} or rendering from interacting meshes~\cite{zhang2024hoidiffusion}.

Our framework is distinguished from these approaches in two key aspects. First, we generate dynamic \textbf{videos} of hand-object interaction, capturing actions rather than the static images produced by prior work. Second, the generated hand motions are \textbf{grounded by an input glove video}. This physical grounding provides precise controllability over the action and enables scalable data curation without requiring object meshes, which are difficult to obtain for non-rigid objects. Furthermore, this approach facilitates the fusion of the generated video with other sensing modalities from the sensor glove.

% \noindent\textbf{Video-to-Video Translation.} Early image-to-image translation methods learned mappings from aligned~\cite{isola2017image} or unpaired~\cite{zhu2017unpaired} image sets. While effective for style transfer, they are not designed for the large physical embodiment differences in our task. Recent video translation works~\cite{yang2023rerender, hu2023videocontrolnet, yang2024fresco, chu2024medm, bian2025videopainter} often rely on latent space interpolation in pre-trained image diffusion models. In contrast, our method learns a direct glove-to-hand video translation from unpaired data, dealing with a significant domain gap, and is not constrained by the capabilities of an existing model.

% \noindent\textbf{Video Inpainting.} A primary goal of video inpainting is object removal and background completion, often using optical flow to propagate information across frames~\cite{zhou2023propainter, li2025diffueraser}. Recent methods leverage diffusion models to inpaint different objects based on language conditions~\cite{ju2024brushnet, yu2023inpaint, gu2024coherent}. Our work is distinct in its focus on inpainting highly detailed hand and object contact regions. The dexterous nature of hands makes this a particularly challenging sub-problem.

% \noindent\textbf{Hand Datasets with Tactile Sensing.} Several datasets capture hand-object interactions~\cite{banerjee2025hot3d, liu2022hoi4d, wang2024ho, fan2023arctic}. ContactPose~\cite{brahmbhatt2020contactpose} estimates binary contact labels by computing distances between reconstructed hand fingertips and object meshes, a practice later adopted by H2O~\cite{kwon2021h2o} and ARCTIC~\cite{fan2023arctic}. PressureVision and EgoPressure~\cite{grady2022pressurevision, grady2024pressurevision++, zhao2025egopressure} provide continuous fingertip force, but it is measured by pressing a Sensel tablet~\cite{senselpad}, which is not suitable for dexterous manipulation. VTacO~\cite{xu2023visual} presents a simulation environment that synthesizes tactile signals for hand-object interactions.
% Kaiwu~\cite{jiang2025kaiwu} provides whole-hand force sensing but is a glove-only dataset. In contrast, our work provides tactile and IMU data from gloves, synchronized with photorealistic interaction videos. To our knowledge, this is the first dataset combining bare-hand videos of dexterous manipulation with sensor-measured tactile and IMU signals.


\noindent\textbf{Video-to-Video Translation.} Early image-to-image translation methods learned mappings from aligned~\cite{isola2017image} or unpaired~\cite{zhu2017unpaired} sets, but are not designed for the large  embodiment differences in our task. Recent video translation works~\cite{yang2023rerender, hu2023videocontrolnet, yang2024fresco, chu2024medm, bian2025videopainter} often rely on latent space interpolation in pre-trained image diffusion models. In contrast, our method learns a direct glove-to-hand video translation from unpaired data, addressing a significant domain gap without being constrained by a pre-trained model's capabilities.

\noindent\textbf{Video Inpainting.} Video inpainting traditionally focused on object removal and background completion, often using optical flow for temporal consistency~\cite{zhou2023propainter, li2025diffueraser}. More recent methods leverage diffusion models for language-conditioned inpainting~\cite{ju2024brushnet, yu2023inpaint, gu2024coherent}. Our work is distinct in its focus on inpainting highly detailed hand-object contact regions, a particularly challenging sub-problem due to the dexterity of hands and the complexity of contact physics.

\noindent\textbf{Hand Datasets with Tactile Sensing.} Datasets for hand-object interaction~\cite{banerjee2025hot3d, liu2022hoi4d, wang2024ho} often estimate binary contact from meshes~\cite{brahmbhatt2020contactpose, kwon2021h2o, fan2023arctic}. While some provide continuous force, they are often limited to flat tablets (restricting dexterity)~\cite{grady2022pressurevision, grady2024pressurevision++, zhao2025egopressure, senselpad}, are simulation-based~\cite{xu2023visual}, or are glove-only datasets lacking visual data~\cite{jiang2025kaiwu}. To our knowledge, our work contributes the first dataset combining sensor-measured tactile and IMU signals with synchronized, photorealistic bare-hand videos of dexterous manipulation.

